UniFlex: Accelerating Networking Research and Experimentation through Software-Defined Wireless Networking

Classical control and management plane for computer networks is addressing individual parameters of protocol layers within an individual wireless network device. We argue that this is not sufficient in phase of increasing deployment of highly re-configurable systems, as well as heterogeneous wireless systems co-existing in the same radio spectrum which demand harmonized, frequently even coordinated adaptation of multiple parameters in different protocol layers (cross-layer) in multiple network devices (cross-node). We propose UniFlex, a framework enabling unified and flexible radio and network control. It provides an API enabling coordinated cross-layer control and management operation over multiple network nodes. The controller logic may be implemented either in a centralized or distributed manner. This allows to place time-sensitive control functions close to the controlled device (i.e., local control application), off-load more resource hungry network application to compute servers and make them work together to control entire network. The UniFlex framework was prototypically implemented and provided to the research community as open-source. We evaluated the the framework in a number of use-cases, what proved its usability.

==> sections/backup_related_work.tex <==
%!TEX root = ../main.tex

\chapter{Related Work}

This section summarizes the most relevant work on this field which falls into three categories:

%
%
%
\section{Cross-layer Coordination}

Akta{\c{s}} et al. proposed CRAWLER~\cite{aktacs2014framework,aktas2012crawler} experimentation architecture for system monitoring and cross-layer coordination for usage in in real testbeds. It offers a centralized control across protocol layers on different devices. In contrast, UniFlex is more flexible as it allows distributing control logic over multiple nodes so that time sensitive control logic can be executed directly on the network node to be controlled.

In~\cite{scheidgen2012clickwatch} we presented the ClickWatch framework which aims to simplify experimentation of wireless cross-layer solutions implemented using the Click Modular Router framework~\cite{kohler2000click}. The basic idea is to observe network nodes in real time in order to create a centralized close to real-time representation of the current network state. Transformation techniques (such as XSL transformations) or specific API allow analyzing the dynamic network state. Based on the observed state the protocol stack of network nodes is reconfigured at real-time. ClickWatch is limited to centralized control.

%
%
%
\section{Software-defined Wireless Networking}

There are already lots of distributed control frameworks, but they are mostly focused on control of wired switches using open protocols (e.g. OpenFlow). Some of them, like ONOS~\cite{berde2014onos} and ONIX~\cite{onix} are focused on scalability and performance. As they are already in very advanced state, it is hard to use them for resource constrained devices or to adjust them for wireless technologies.

Ryuo~\cite{ryuo} is an extension of the very popular Ryu controller. Ryuo uses local services that run on the SDN switches and serve most frequent events, thus limiting control traffic volume between switch and global controller. Therefore, local services provide a high level northbound API to global Ryuo applications.

Kandoo~\cite{hassas2012kandoo} is comparable with Ryuo as it also provides the possibility for offloading of control applications as way to limit the control plane load. Therefore, Kandoo introduces two levels of controllers. Local controllers handle frequent events, while a logically centralized root controller handles rare events. In contrast to Kandoo, UniFlex is not restricted to two levels of controllers as it allows direct communication between any controller applications. Moreover, Kandoo is focused on wired networks.

Beehive~\cite{beehive1}\cite{beehive2} is distributed framework that is able to automatically compile applications into their distributed counterparts and optimize placement of functions between nodes in network at run-time. Functions are able to communicate by means of exchanging events and by sharing state using dictionaries. The Beehive framework guarantee to execute functions that share state in single thread in order to avoid race-conditions and assure consistency. Based on Beehive, authors were able to implement SDN controller for network of wired switches. While having couple of similar concepts, Beehive does not differentiate between control applications and device modules as Uniflex. 
%Moreover, there is no unification of NDPI of heterogenous devices. 

CoAP~\cite{patro2015coap} proposes a vendor neutral centralized framework for configuration, coordination and management of residential 802.11 APs using an open API implemented over the OpenFlow~\cite{mckeown2008openflow} SDN framework. In contrast to UniFlex the CoAP API is restricted to WiFi networks. Moreover, only centralized control programs are possible.

OpenRF~\cite{kumar2013bringing} follows the design principle of OpenFlow by separating the data and control plane. However, unlike OpenFlow which remains at Layer-2, OpenRF provides programming abstractions tailored for wireless networks, i.e. MIMO interference management techniques that impact the physical layer. OpenRF is restricted to centralized control of WiFi infrastructure networks.

Riggio et al.~\cite{riggio2015programming} proposed a set of programming abstractions for wireless networks targeting four control aspects, namely, state management, resource allocation, network monitoring and reconfiguration. While it greatly simplifies the development of network apps we believe that the device module concept of UniFlex is more flexible allowing to adapt to future device functionality, i.e. missing functionality can be easily added by extending the API. Note, the key abstractions from~\cite{riggio2015programming} like Light Virtual Access Point and Wireless Termination Point can be implemented as UniFlex network apps.

In \cite{zubow2015sdn} we proposed architecture for centralized spectrum brokerage in residential infrastructure Cognitive Radio networks using SDN principles. A cloud-based controller decides on spectrum allocation by taking into account network topology information, traffic and channel conditions.% It can be implemented as UniFlex network app.

%
%
%
\section{Distributed Control Platforms}

ROS~\cite{quigley2009ros} is an open source robot operating system for rapid prototyping. It is motivated by the variety of different types of robots each with different hardware. In ROS a node does not expose its devices outside. Instead it exposes topics, on which it listens for commands. Node implements functions that are executed on devices. 
%\mcf{Both are in many cases very simmilar. ROS is much more mature, and has a lot more support for the task at hand (controlling robots of any kind). They don't have time scheduled execution of tasks. They don't have the concept of multiple physical nodes doing the same}
% ROS doesn't have discovery, you have to provide where is master node, otherwise it will not work. It also requires IP connectivity between all ros nodes (P2P connections, without proper routing ROS breaks)
ROS is focused on providing a control for one robot, trying to achieve one goal, and having all nodes working towards that goal. In UniFlex, we are trying to achieve harmonization of multiple devices. We also provide time scheduled execution of the same task on multiple devices that ROS doesn't support (and doesn't need).

%TANGO~\cite{gotz2003tango} is the most common control systems used in the synchrotron community. It provide hardware-independent and distributed access to a variety of devices. However, it does not provide a high-level device and process control API.

==> sections/extension.tex <==
%!TEX root = ../main.tex

\section{How to extend UniFlex?}

The core (middle-ware) of the framework as well as multiple device modules and couple of example controllers are provided to research community as open-source using MIT licence. 

\tolja{Very each - Scripting in high-level language - Python}

\subsection{How to add a new UPI function/event?}

\tolja{TBD. Write interface in module upis and add implementation to corresponding device abstraction class.}

\subsection{How to add new device abstraction class?}

\tolja{TBD. Write Python module + add it to yaml config.}

==> sections/trash.tex <==
\subsection{Rules}

In the past few years, the "mach+action" abstraction is widely used for packet forwarding in Software-Defined-Networks. Our idea is to adopt such an approach for implementation of reactive control in $\text{C}^\text{3}$ framework. The Rules are building blocks that allow for writing simple control programs. In general, rule consist of Data Source, list of Filters, Condition and list of Actions that are executed whenever condition is matched --- Fig.~\ref{fig:rule}. Only a Data Source object is required to setup new rule and the others are optional. In such case, rule is simply a source of streaming data. The Data Source is a source of stream of data, where the stream is generated using UPI.

While in case of UPI events and services, their output is already a stream of data, in case of UPI functions additional mechanisms are required to generate stream. Here, we propose event driven execution of UPI functions. Currently, we support two kinds of events: time-based event and packet-based event. The former one is simply repeating execution of UPI function with specified frequency, while in latter one UPI calls are triggered on packet arrival event. 
The list of filters may be applied to stream of data generated in Data Source. Simple filters like moving average or peak detector are provided. They take numerical value as input and give numerical output. We are aware that this is not always a case, that Data Source generate numerical stream, thus we leave a developers a possibility to inherit from base Filter class and implement their own filter. 

The filtered data stream is an input to Condition block. If the condition is met, a signal to fire all registered Actions is generated. The rule may be removed just after first N matches. We call it then \emph{transient rule}. If decision when to remove a rule do not depend on number of times it was matched, it is called \emph{persistent rule}.

The rules are fully executed in agent. They may be considered as small control programs injected by control program into agent. This allows us not only to distribute processing of data, but also save resources on communication channel between controller and agent.

The API that allows to manage rules contains two functions: \emph{install\_rule()}, that returns rule ID (descriptor) and \emph{delete\_rule()}, that takes rule ID (descriptor) as a parameter.  

\begin{figure}[!ht]
   \begin{center}
       \includegraphics[width=0.8\linewidth]{figs/rule_concept}
   \end{center}
    \vspace{-10pt}
   \caption{Structure of $\text{C}^\text{3}$ Rule}
   \label{fig:rule}
\end{figure}




Node contains devices and applications
Controller implemented as distributed and cooperating applications
devices expose set of operations and signals
device interface is southbound interface
northbound interface allow to access SB interface of any device in any control application

applications talk to each other by means of exchanging events that are coupled with functions 
events are asynchronous messages that trigger functions
function may further generate new events
application may store state inside

function chaining 
functions inside one application may share state
Functions of two different applications communicate using messages and cannot share state
description set of operation of devices
